Curvature-Independent Regret Bounds for Distributed Online Optimization on Hadamard Manifolds

This work addresses decentralized online Riemannian optimization on Hadamard manifolds. Prior work under geodesic convexity (g-convexity) may require curvature information in the optimization analysis, typically through a finite lower bound on the sectional curvature. Curvature may also enter the step size or contraction factor of tangent-space Riemannian consensus schemes. In this work, we relax the curvature dependence for a narrower class of horospherical convex (h-convex) functions. We study Distributed Riemannian Online Gradient Descent (D-ROGD), which combines local Riemannian h-subgradient updates with an implicit Fr\'echet-mean consensus. For h-convex and strongly h-convex local objectives, we establish $O(\sqrt{T})$ and $O(\log T)$ static regret, respectively, matching the corresponding Euclidean rates with respect to $T$, with network dependence governed solely by the spectral gap. To our knowledge, these are the first curvature-independent regret guarantees for decentralized online optimization on Hadamard manifolds. Experiments on hyperbolic embeddings corroborate the predicted rates, with no observable degradation due to curvature.

==> arguments.tex <==

Some arguments:
\begin{itemize}
\item 
\item In Euclidean space, the fact that geodesic and horospherical convexity coincide is the central tool of convex analysis: the supporting hyperplane theorem. By
contrast, in the case of hyperbolic space, for compact sets with nonempty interior, horospherical convexity entails a certain level of curvature in the boundary,
and is a strictly stronger property than geodesic convexity \cite{lewis2024horoballs}.
\item Our complexity analysis is geometrically appealing: like the algorithm itself, it makes no use of
tangent spaces, and as we have noted, applies to objectives that may be nonconvex
but have horospherically convex level sets \cite{lewis2024horoballs}.

\item The algorithm does not apply to every geodesically convex objective, but its range
of application is still rich. Furthermore, our complexity result involves no lower
curvature bound, so even applies in spaces with infinite negative curvature and
bifurcating geodesics, such as the tree spaces and cubical complexes of [1, 8].

\item Busemann functions are 1-Lipschitz and convex, and their lower level sets are
called horoballs \cite{lewis2024horoballs}.

\item When comparing h-convexity and g-convexity, h-convexity generalizes the outer and global aspects of convexity, while g-convexity generalizes the inner and local aspects of
convexity \cite{criscitiello2025horospherically}.

\item h-subdiff is a subset of g-subdiff Prop2,iii \cite{criscitiello2025horospherically}.

\item This in turn means that
gradient descent based on geodesic smoothness takes much smaller step sizes than gradient descent based on horospherical smoothness

\item $y \mapsto d(y,p)$ is $h$-convex so we can use this in experiments.


\end{itemize}
